Thought Bubbles: A Proxy into Players' Mental Model Development

Studying mental models has recently received more attention, aiming to understand the cognitive aspects of human-computer interaction. However, there is not enough research on the elicitation of mental models in complex dynamic systems. We present Thought Bubbles as an approach for eliciting mental models and an avenue for understanding players' mental model development in interactive virtual environments. We demonstrate the use of Thought Bubbles in two experimental studies involving 250 participants playing a supply chain game. In our analyses, we rely on Situation Awareness (SA) levels, including perception, comprehension, and projection, and show how experimental manipulations such as disruptions and information sharing shape players' mental models and drive their decisions depending on their behavioral profile. Our results provide evidence for the use of thought bubbles in uncovering cognitive aspects of behavior by indicating how disruption location and availability of information affect people's mental model development and influence their decisions.

==> sections/07_conclusion.tex <==
% \section{Conclusion}
% In this paper, we presented an approach called \textit{thought bubbles} for eliciting mental model development of players' in their interaction with a dynamic virtual environment. We demonstrated how we designed thought bubbles to evoke players' thinking and collect qualitative data on their thought processes diegetically and temporally. We showed a mixed-method approach for analyzing elicited mental models by grounding our qualitative analysis the Situation Awareness model to gain a theoretical understanding of cognitive aspects of human decisions and their mental model formation. Using thought bubbles, we studied players' mental model development over time in two experimental studies in the context of supply chains. We provided evidence for the value of thought bubbles by showing how disruption location and supply chain information sharing affects the formation of mental models 

% Our work particularly a
